INSIGHT: Enhancing Autonomous Driving Safety through Vision-Language Models on Context-Aware Hazard Detection and Edge Case Evaluation

Autonomous driving systems face significant challenges in handling unpredictable edge-case scenarios, such as adversarial pedestrian movements, dangerous vehicle maneuvers, and sudden environmental changes. Current end-to-end driving models struggle with generalization to these rare events due to limitations in traditional detection and prediction approaches. To address this, we propose INSIGHT (Integration of Semantic and Visual Inputs for Generalized Hazard Tracking), a hierarchical vision-language model (VLM) framework designed to enhance hazard detection and edge-case evaluation. By using multimodal data fusion, our approach integrates semantic and visual representations, enabling precise interpretation of driving scenarios and accurate forecasting of potential dangers. Through supervised fine-tuning of VLMs, we optimize spatial hazard localization using attention-based mechanisms and coordinate regression techniques. Experimental results on the BDD100K dataset demonstrate a substantial improvement in hazard prediction straightforwardness and accuracy over existing models, achieving a notable increase in generalization performance. This advancement enhances the robustness and safety of autonomous driving systems, ensuring improved situational awareness and potential decision-making in complex real-world scenarios.

==> sec/prelim.tex <==



\section{Preliminaries}
\label{sec:prelim}
\subsection{Transformer \& LLM Basics}
Large language models (LLMs) are decoder-style Transformers trained with self-supervision to model token sequences. At inference, they generate text autoregressively: the next token is predicted from the context.

\subsubsection{Multi-Head Attention}
Given tokens $\mathbf{X}\!\in\!\mathbb{R}^{L\times d}$, each head $h\!\in\!\{1,\dots,H\}$ computes
\begin{equation}
\mathbf{Q}_h=\mathbf{X}\mathbf{W}^Q_h,\quad
\mathbf{K}_h=\mathbf{X}\mathbf{W}^K_h,\quad
\mathbf{V}_h=\mathbf{X}\mathbf{W}^V_h,
\end{equation}
with $\mathbf{W}^{Q/K/V}_h\!\in\!\mathbb{R}^{d\times d_h}$ and $d_h=d/H$. Scaled dot-product attention is
\begin{equation}
\mathrm{Attn}_h(\mathbf{X})=\mathrm{softmax}\!\left(\frac{\mathbf{Q}_h\mathbf{K}_h^\top}{\sqrt{d_h}}+\mathbf{M}\right)\mathbf{V}_h,
\end{equation}
where $\mathbf{M}\!\in\!\mathbb{R}^{L\times L}$ is an additive mask (e.g., $0$ for allowed, $-\infty$ for disallowed). The multi-head output is
\begin{equation}
\mathrm{MHSA}(\mathbf{X})=\mathrm{Concat}\!\big(\mathrm{Attn}_1,\ldots,\mathrm{Attn}_H\big)\mathbf{W}^O,\quad \mathbf{W}^O\!\in\!\mathbb{R}^{(Hd_h)\times d}.
\end{equation}
Transformers use residual connections and LayerNorm around MHSA and a position-wise feed-forward network (FFN).

\subsubsection{Causal vs.\ Bidirectional Masks}
Causal masks restrict a position to attend only to itself and prior positions (used for generation). Bidirectional masks allow full attention within a set of tokens (used for non-autoregressive blocks, e.g., visual tokens).

% ------------------------ ViT ------------------------
\subsection{Vision Encoder (ViT) Basics}
A Vision Transformer (ViT) splits an image into fixed-size patches, projects each patch to an embedding, and applies self-attention to model global context.

\paragraph{Patch Embedding and 2D-RoPE.}
Patch embeddings form a sequence; 2D rotary position embeddings (2D-RoPE) inject height/width structure to preserve spatial locality.

\paragraph{Token Compression \& Dynamic Resolution (Packing).}
To control sequence length and memory, adjacent visual tokens may be merged by a lightweight MLP, and images are dynamically resized within pixel bounds so multiple images can be packed into one sequence before fusion.

% ------------------------ Positional Encoding ------------------------
\subsection{Positional Encoding}
\paragraph{RoPE.} Rotary position embedding (RoPE) encodes positions by rotating query/key vectors with frequency-based phases (standard 1D for text).
\paragraph{2D-RoPE.} Extends RoPE to two spatial axes (height, width) for images in the vision encoder.
\paragraph{M-RoPE.} Multimodal RoPE decomposes positional signals along time/height/width for unified text–image(/video) modeling in the decoder.

% ------------------------ Fusion ------------------------
\subsection{Multimodal Fusion in VLMs}
VLMs combine visual and textual tokens for joint reasoning.

\subsubsection{Early Fusion (Qwen2-VL)}
Visual tokens are placed before text and delimited by special markers (e.g., $vision\_start$, $vision\_end$). The concatenated sequence is fed to the decoder-only LLM. The decoder uses MHSA with M-RoPE so each text position can attend to all visual tokens and past text while generating.

\subsubsection{Late Fusion (Cross-Attention) and Hybrid}
Late fusion queries fixed visual features with cross-attention (\(\mathbf{Q}\) from text; \(\mathbf{K},\mathbf{V}\) from vision), reducing compute at generation time. Hybrid designs mix early fusion at selected layers with cross-attention elsewhere.

\subsubsection{Mixed Masking \& Vision Segment Markers}
A mixed mask is applied: (i) visual$\leftrightarrow$visual tokens attend bidirectionally; (ii) text tokens are causal and may attend to all visual tokens and prior text; (iii) optional blocking of vision$\rightarrow$text prevents leakage of future text. Vision segment markers help the model localize visual spans within the joint sequence.


